Exploring the Frontiers of Energy Efficiency using Power Management at System Scale

In the face of surging power demands for exascale HPC systems, this work tackles the critical challenge of understanding the impact of software-driven power management techniques like Dynamic Voltage and Frequency Scaling (DVFS) and Power Capping. These techniques have been actively developed over the past few decades. By combining insights from GPU benchmarking to understand application power profiles, we present a telemetry data-driven approach for deriving energy savings projections. This approach has been demonstrably applied to the Frontier supercomputer at scale. Our findings based on three months of telemetry data indicate that, for certain resource-constrained jobs, significant energy savings (up to 8.5%) can be achieved without compromising performance. This translates to a substantial cost reduction, equivalent to 1438 MWh of energy saved. The key contribution of this work lies in the methodology for establishing an upper limit for these best-case scenarios and its successful application. This work sheds light on potential energy savings and empowers HPC professionals to optimize the power-performance trade-off within constrained power budgets, not only for the exascale era but also beyond.

==> Makefile <==
#
# Makefile for acmart package
#
# This file is in public domain
#
# $Id: Makefile,v 1.10 2016/04/14 21:55:57 boris Exp $
#

all: sc21

.PHONY: sc21
sc21: sc21.pdf	

sc21.pdf: ./txt/*.tex ./figs/*
	pdflatex sc21.tex
	- bibtex sc21
	pdflatex sc21.tex
	- bibtex sc21
	pdflatex sc21.tex

docclean:
	$(RM)  *.log *.aux \
	*.cfg *.glo *.idx *.toc \
	*.ilg *.ind *.out *.lof \
	*.lot *.bbl *.blg *.gls *.cut *.hd \
	*.dvi *.ps *.thm *.tgz *.zip *.rpi \
	*.fdb_latexmk \
	*.synctex.gz

clean: docclean
	$(RM) sc21.pdf
	

.PHONY: all docclean clean


==> figs/all_class.tex <==
\begin{figure}[t]
  \centering

  \includegraphics[width=\linewidth]{figs/all_class1.pdf}
    %\caption{Example plot}
    \caption{Groupings of power profiles based on the power utilization patterns exhibited by jobs. The different classes can be grouped into high-level classification into three types. Classes from 0-20 are compute intensive, 21-92 are mixed type, and 93-118 are non-compute intensive jobs. Tiles with blue curve have high power consumption and plots with green curve have low power consumption.  Intensity of the background color of each tile represents the density of each pattern among the entire population.}
  \label{fig:all_class}
\end{figure}


==> figs/workflow.tex <==
%% Template for a page-wide figure
\begin{figure*}[t]
  \centering
  \includegraphics[width=18cm, height=3cm]{figs/template_wide.pdf}
  \caption{Workflow pipeline describing the overview of the energy projection pipeline}
  %\description{Description of the image}
  \label{figs:workflow}
\end{figure*}


==> plots/projection_plot.tex <==
\begin{figure}[t]
  \centering
  \includegraphics[width=\linewidth]{plots/template_single.pdf}
    \caption{Saving projection graph.}
  \label{plots:saving-projection}
\end{figure}


==> plots/roofline_plot_compute_vs_bandwidth.tex <==
\begin{figure}[t]
  \centering
  \includegraphics[width=\linewidth]{plots/template_single.pdf}
    \caption{Replaced:Workflow End-to-end. /Roofline plot of Bandwidth vs Compute for Summit and Frontier GPUs}
  \label{plots:example}
\end{figure}


==> plots/three_class_wrokloads.tex <==
\begin{figure}[t]
  \centering
  \includegraphics[width=\linewidth]{plots/classes_groups.pdf}
    \caption{(\textbf{Will add a similar Figure from Froniter jobs})Three different type of workloads a) Compute intensive, b) Non-compute intensive, and c) Mixed of compute and non-compute workloads.}
  \label{plots:3-class}
\end{figure}


==> plots/understanding_gpu_operation.tex <==
\begin{figure}[t]
  \centering
  \includegraphics[width=\linewidth]{plots/template_single.pdf}
    \caption{Plot for high level trend in GPU operations.}
  \label{plots:understanding-workloads}
\end{figure}


==> tables/evaluation.tex <==
% \begin{table}
%     \caption{Cluster Homogeneity}
%   \label{tab:eval}
%   %% Footnotesize if a much smaller font is needed
%   \footnotesize
%   \begin{tabular}{lccccc}
%     \toprule
%       Exp. & Method & L1(\%) & L2(\%) & L3(\%) & L4(\%)\\
%     \midrule
%     \multirow{2}{*}{Main} & KMeans & 90.4 & 85.5 & 75.5 & 70.1\\
%                          & DBSCAN & raw data & 12 months & A &\\
%     \multirow{2}{*}{Baseline} & KMeans & raw data & 12 months & A &\\
%                          & DBSCAN & raw data & 12 months & A &\\
%   \bottomrule
% \end{tabular}
% \end{table}

\begin{table}
    \caption{Cluster homogeneity}
  \label{tab:eval_cluster_homogenety}
  %% Footnotesize if a much smaller font is needed
  \footnotesize
  \begin{tabular}{ccccc}
    \toprule
      Method & L1(\%) & L2(\%) & L3(\%) & L4(\%)\\
    \midrule
    KMeans & 90.4 & 85.5 & 75.5 & 70.1\\
    DBSCAN & 84.2 & 78.2 & 74.4 &69.7\\
  \bottomrule
\end{tabular}
\end{table}
\vspace{-2pt}

==> txt/06_related.tex <==

\section{Related Works}
\label{sec:relatedWorks}


\woong()
\loremipsum{\textbf{100-words}
odio eu feugiat pretium nibh ipsum consequat nisl vel pretium lectus quam id leo in vitae turpis massa sed elementum tempus egestas sed sed risus pretium quam vulputate dignissim suspendisse in est ante in nibh mauris cursus mattis molestie a iaculis at erat pellentesque adipiscing commodo elit at imperdiet dui accumsan sit amet nulla facilisi morbi tempus iaculis urna id volutpat lacus laoreet non curabitur gravida arcu ac tortor dignissim convallis aenean et tortor at risus viverra adipiscing at in tellus integer feugiat scelerisque varius morbi enim nunc faucibus a pellentesque sit amet porttitor eget dolor morbi non arcu risus}

\loremipsum{\textbf{100-words}
odio eu feugiat pretium nibh ipsum consequat nisl vel pretium lectus quam id leo in vitae turpis massa sed elementum tempus egestas sed sed risus pretium quam vulputate dignissim suspendisse in est ante in nibh mauris cursus mattis molestie a iaculis at erat pellentesque adipiscing commodo elit at imperdiet dui accumsan sit amet nulla facilisi morbi tempus iaculis urna id volutpat lacus laoreet non curabitur gravida arcu ac tortor dignissim convallis aenean et tortor at risus viverra adipiscing at in tellus integer feugiat scelerisque varius morbi enim nunc faucibus a pellentesque sit amet porttitor eget dolor morbi non arcu risus}

==> txt/artifact_description.tex <==

\section{Artifact Description}
\setcounter{table}{0}
\renewcommand{\thetable}{A\arabic{table}}
%\renewcommand{\thesubsection}{\arabic{subsection}}

\subsection{Artifact Identification}
%START_LATEX
\textbf{Title}: Machine Learning Assisted Profiling of Jobs Power Consumption Timeseries for Large Scale HPC System\\
\textbf{Authors}: Ahmad Maroof Karimi, Naw Safrin Sattar, Woong Shin, Feiyi Wang \\
\textbf{Affiliation}: Oak Ridge National Laboratory\\
\\
The main contribution of the paper is the data-driven end-to-end pipeline designed and developed for processing, managing, and classification of power profiles of the system-wide workloads of a large-scale HPC system. 
Major tasks accomplished by the end-to-end workflow pipeline shown in Figure 2 of the paper are: 1) power \& energy and jobs data collection, 2) processing raw data, 3) storing the processed data in the low latency distributed database, 4) feature extraction, 5) latent feature generation 6) hierarchical classification labeling, and 7) calculating clustering and prediction quality. A brief description of the tasks is as follows:

\begin{itemize}
	\item Data Collection: We collect raw compute-node level power data and job scheduler logs; collected logs for all the workloads in the year 2021, consisting of over 1.5 million jobs (shown in Table 1 of the article).
	\item Data processing: In this stage, raw power and energy data, which is system-level data, is synced with application-level jobs logs. The processed data are listed in Table 2 in the paper.
    \item Data storage: For low latency and high availability of timeseries data, we used the Apache Druid database to store all the processed data, described in Table 2 of the paper.
	\item Features extraction: The processed data is 10 sec—interval timeseries for every job. Thus the length of the timeseries depends on the duration for which the job ran. In the feature extraction step, we extract features related to magnitude and swings/changes in the timeseries. We have summarized the list of features we extracted in Table 3 of the paper. This appendix presents the feature list with a more detailed description in Table \ref{tab:ftr_apndx_tbl}.
    \item Latent feature generation: Latent feature generation using the GAN model has several advantages in the analysis and modeling of the power profiles. We have leveraged it here to reduce the dimensionality of the feature set to enable better clustering scores.
	\item Hierarchical classification labeling: The significance of this task is to enable us to validate and assess the quality of the machine learning methods we used. Although we processed and performed clustering of about 60K jobs, we labeled 846 random samples to calculate and report the cluster quality and prediction quality in this task. As described in Section 4.4 of the paper, we did hierarchical labeling in four levels (L1, L2, L3, and L4). Hierarchical labels enabled us to look at the power patterns exhibited by jobs at multiple granularities. A summary of the classification label is shown in Table 4 of the article. Table~\ref{tab:class_level_labels} shows the number of high-level classes at L1 and subclasses at levels L2 L3, and L4. 
    \item Clustering and Prediction: We identify and classify power profiles exhibited by HPC jobs into different classes at different resolution levels. The clustering and prediction quality scores are reported in sections 5.1 and 5.2, respectively.
    \end{itemize}

While the primary artifact is essentially an end-to-end data pipeline, artifacts resulting from this work also include a framework and a set of infrastructure-level building blocks dedicated for use to support such a data pipeline.
Implemented in the forms of in-house re-usable python libraries, the framework supports data pipeline artifacts which are implemented and deployed as either containerized persistent applications or a workflow, connecting and orchestrating several infrastructure-level building blocks we have deployed for this work.  These building blocks provide the ability to efficiently utilize the necessary compute, memory, and storage while handling large volumes of data involved.  Mainly depicted in Figures 2 and 3 in Section 3, such infrastructure-level building blocks include the following:

\begin{itemize}
    \item Minio, an S3 interface-based object storage to store archived historical data or intermediate data for batch processing as well as providing backend persistence for other building blocks
    \item Apache Druid, a timeseries database to serve downstream interactive workloads via REST APIs or web applications
    \item Apache Spark-based data analytics cluster for both batch and stream data processing
    \item MLFlow, an experiment tracker and model registry for machine learning model development and maintenance
    \item Apache Airflow, a workflow orchestration engine to perform batch processing orchestration of workflows
    \item RedisAI, an inference server for GPU usage consolidation for online inference
    \item Jupyterhub, a multi-tenent jupyter notebook server provider to support the interactive needs of the authors in developing and managing the data pipelines and experiments
\end{itemize}

The artifacts of this work include a wide array of components required for high-performance data processing and data-intensive machine learning modeling tasks.  However, the system still relies on several external systems and services provided to the authors from other groups in our organization. These systems and services are not scoped as artifacts from this work. Such items are as the following:

\begin{itemize}
    \item Center-wide Kubernetes cluster which all the artifacts are deployed and operated on top of
    \item The data engineering and distribution system depicted in Figure 1 provides a unified interface to a wide array of data streams coming from heterogeneous data sources
\end{itemize}

The computational artifacts (dataset and workflow pipeline/code) have a major role in enabling us to develop a system for profiling and classifying power profiles of all workloads on the HPC machine. The results presented in the paper are the direct outcome of the workflow presented here. 

\begin{table}
    \caption{Features extracted from timeseries of power profiles of each job. The features prefixed with $1\_$ represent the features calculated for the first bin. We similarly calculate features for the other three bins, not shown here for brevity. The four bins are created by partitioning the timeseries into 4 parts across the length of the timeseries}
    \label{tab:ftr_apndx_tbl}
    \footnotesize

    \begin{tabular}{ll}
        \toprule
        Features & Description \\
        \midrule
        allocation\_id & jobs allocation id \\
        total\_mean & mean input power of full timeseries \\
        length & length of the timeseries \\
        1\_mean\_inp\_power & mean input power \\
        1\_median\_inp\_power & median input power \\
        1\_sfqp\_25\_50 & no. of up swings from 25 to 50W \\
        1\_sfqn\_25\_50 & no. of down swings from 25 to 50W \\
        1\_sfql2p\_25\_50 & no. of up swings from 25 to 50W over 2 time-period \\
        1\_sfql2n\_25\_50 & no. of down swings from 25 to 50W over 2 time-period \\
        1\_sfqp\_50\_100 & no. of up swings from 50 to 100W \\
        1\_sfqn\_50\_100 & no. of down swings from 50 to 100W \\
        1\_sfql2p\_50\_100 & no. of up swings from 50 to 100W over 2 time-period \\
        1\_sfql2n\_50\_100 & no. of down swings from 50 to 100W over 2 time-period \\
        1\_sfqp\_100\_200 & no. of up swings from 100 to 200W \\
        1\_sfqn\_100\_200 & no. of down swings from 100 to 200W \\
        1\_sfql2p\_100\_200 & no. of up swings from 100 to 200W over 2 time-period \\
        1\_sfql2n\_100\_200 & no. of down swings from 100 to 200W over 2 time-period \\
        1\_sfqp\_200\_300 & no. of up swings from 200 to 300W \\
        1\_sfqn\_200\_300 & no. of down swings from 200 to 300W \\
        1\_sfql2p\_200\_300 & no. of up swings from 200 to 300W over 2 time-period \\
        1\_sfql2n\_200\_300 & no. of down swings from 200 to 300W over 2 time-period \\
        1\_sfqp\_300\_400 & no. of up swings from 300 to 400W \\
        1\_sfqn\_300\_400 & no. of down swings from 300 to 400W \\
        1\_sfql2p\_300\_400 & no. of up swings from 300 to 400W over 2 time-period \\
        1\_sfql2n\_300\_400 & no. of down swings from 300 to 400W over 2 time-period \\
        1\_sfqp\_400\_500 & no. of up swings from 400 to 500W \\
        1\_sfqn\_400\_500 & no. of down swings from 400 to 500W \\
        1\_sfql2p\_400\_500 & no. of up swings from 400 to 500W over 2 time-period \\
        1\_sfql2n\_400\_500 & no. of down swings from 400 to 500W over 2 time-period \\
        1\_sfqp\_500\_700 & no. of up swings from 500 to 700W \\
        1\_sfqn\_500\_700 & no. of down swings from 500 to 700W \\
        1\_sfql2p\_500\_700 & no. of up swings from 500 to 700W over 2 time-period \\
        1\_sfql2n\_500\_700 & no. of down swings from 500 to 700W over 2 time-period \\
        1\_sfqp\_700\_1000 & no. of up swings from 700 to 1000W \\
        1\_sfqn\_700\_1000 & no. of down swings from 700 to 1000W \\
        1\_sfql2p\_700\_1000 & no. of up swings from 700 to 1000W over 2 time-period \\
        1\_sfql2n\_700\_1000 & no. of down swings from 700 to 1000W over 2 time-period \\
        1\_sfqp\_1000\_1500 & no. of up swings from 1000 to 1500W \\
        1\_sfqn\_1000\_1500 & no. of down swings from 1000 to 1500W \\
        1\_sfql2p\_1000\_1500 & no. of up swings from 1000 to 1500W over 2 time-period \\
        1\_sfql2n\_1000\_1500 & no. of down swings from 1000 to 1500W over 2 time-period \\
        1\_sfqp\_1500\_2000 & no. of up swings from 1500 to 2000W \\
        1\_sfqn\_1500\_2000 & no. of down swings from 1500 to 2000W \\
        1\_sfql2p\_1500\_2000 & no. of up swings from 1500 to 2000W over 2 time-period \\
        1\_sfql2n\_1500\_2000 & no. of down swings from 1500 to 2000W over 2 time-period \\
        1\_sfqp\_2000\_3000 & no. of up swings from 2000 to 3000W \\
        1\_sfqn\_2000\_3000 & no. of down swings from 2000 to 3000W \\
        1\_sfql2p\_2000\_3000 & no. of up swings from 2000 to 3000W over 2 time-period \\
        1\_sfql2n\_2000\_3000 & no. of down swings from 2000 to 3000W over 2 time-period\\
        \bottomrule

    \end{tabular}
\end{table}

\begin{table}
    \caption{The number of classes at different levels of classification. L1 is the highest level of classification, and there are 12 high-level classes.}
    \label{tab:class_level_labels}
    \footnotesize

    \begin{tabular}{cccc}
    \toprule
    L1 & L2 & L3 & L4 \\
    \midrule
    \begin{tabular}[c]{@{}l@{}}High-level\\ classification\end{tabular} & \multicolumn{3}{l}{Sub-classes} \\
    \midrule
    A & 1 & 1 & 1 \\
    B & 1 & 2 & 2 \\
    C & 1 & 2 & 3 \\
    D & 1 & 4 & 4 \\
    F & 5 & 26 & 41 \\
    G & 5 & 14 & 22 \\
    H & 2 & 8 & 12 \\
    J & 2 & 5 & 6 \\
    L & 1 & 1 & 1 \\
    M & 1 & 2 & 3 \\
    N & 1 & 3 & 3 \\
    O & 2 & 2 & 2\\
    \bottomrule
    \end{tabular}
\end{table}
%STOP_LATEX


\subsection{Reproducibility of Experiment}:
%START_LATEX
\subsubsection{Description of the Experiment Workflow}
The end-to-end pipeline shown in Figure 2 represents the major steps involved in the framework. In the data ingestion task, we have collected system-level data and job allocation logs. During the data processing stage, we developed Python based Apache Spark scripts for processing a large amount of data by leveraging Apache Spark's distributed computing techniques for efficient processing.  After data processing, we ingest the processed data into the Apache Druid timeseries database for online interactive consumption, and also into the object store in an archived form (i.e., Apache Parquet files leveraging the Snappy algorithm) for long-term batch processing.
Mainly using the archived data for efficient batch processing, we extracted features from the processed data for a system-wide cross-sectional analysis and modeling of jobs' power profiles. The summarized list of the features is shown in the paper in Table 3. A more descriptive list of features is given here in Table \ref{tab:ftr_apndx_tbl}.
The list of features extracted is fed into the GAN model shown in Figure 5 to generate latent features of size 20. The GAN model helps reduce the dimensionality of the data and simultaneously preserves the information contained in the data. The dimensionally reduced data is used for machine learning tasks such as clustering. 
Although we cluster about 60K jobs, for calculating and reporting cluster quality scores, we labeled 846 jobs. The labeling of datasets enabled us to measure the quality of different methods in absolute numbers instead of clustering metrics such as the Silhouette score. The labeling of the cluster is accomplished at 4 resolution levels. At level-1 or L1, shown in Table 5 in the paper, we classify the datasets into 12 classes. At higher resolutions, such as at levels L2, L3, and L4, the 12 main classes at L1 are further classified into many subclasses. We report the cluster homogeneity scores in section 5.1 of the paper. In another experiment, we partition the labeled dataset into two sets of 80\% and 20\% using scikit-learn stratified-kfold cross-validation method. We use the k-means to cluster on 80\% of the data. Then we use the k-means center to predict the classes or groups of 20\% of the data based on the proximity with the cluster center. We report the results of the homogeneity score on 20\% of the data in section 5.2 of the paper. 
% \begin{itemize}
%     \item Dataset
%     \begin{enumerate}
%         \item Raw Dataset
%         \item Processed Data
%         \item Extracted Features

%     \end{enumerate}
%     \item Workflow
%     \begin{enumerate}
%         \item 
%     \end{enumerate}    
% \end{itemize}


\subsubsection{Execution Time to Execute the Experiment Workflow}
\textit{Data-processing}: The execution time of the initial historical data processing is 3 minutes per day of data. This makes up about 19 hours for a year's worth of data on our Spark cluster using 128-cores and 512GB memory.
\textit{Feature extraction}: The feature extraction step takes about 1 minute per day of data or 6 hours per year.  This task was executed on the Spark environment using 42 cores and 8 GB of memory per executor.
\textit{Latent feature generation by GAN}: Each epoch takes about 40 seconds, and we run it for 1000 epochs needing about 10 hours. The GAN model was developed using Python's pytorch library. The task was executed on single a node having 8GB partition of an Nvidia A100 leveraging its multi-instance GPU feature, 16 CPU cores, and 16 GB memory.  
\textit{Evaluation}7: We filtered and randomly selected 846 jobs and labeled them by hand. Labeled data was used for evaluating clustering and prediction quality. The clustering algorithms and subsequent prediction were performed on a single-node machine in a Python environment using scikit-learn python packages. The evaluation task's overall execution time on 16 cores, 16 GB memory is about 90 seconds. 

\subsubsection{A Complete Description of the Expected Results and Evaluation}
The results generated by the workflow are much more comprehensive than what we reported in the article because of the space constraint. For clustering methods in k-means and DBSCAN, we explored a broad range of search spaces. For k-means, we ran the experiments with a value of K ranging from 60 to 120. Similarly, we ran DBSCAN with different combinations of the two parameters: 1) epsilon values and 2) minimum samples, as shown in Table~\ref{tab:dbscan_grid_search}.
To maintain the repeatability of results for k-means, we fixed the random\_state parameter of the k-means function. For DBSCAN we pass the data in the same order to maintain the deterministic property of the results. 

\begin{table}
    \caption{DBSCAN Grid Search Space}
    \label{tab:dbscan_grid_search}
    \footnotesize

    \begin{tabular}{cc}
    \toprule
    Epsilon & Minimum Samples \\
    
    
    \midrule
0.880 & 5      \\
0.880 & 10     \\
0.880 & 15     \\
0.881 & 5      \\
0.881 & 10     \\
0.881 & 15     \\
0.882 & 5      \\
0.882 & 10     \\
0.882 & 15     \\
0.883 & 5      \\
0.883 & 10     \\
0.883 & 15     \\
0.884 & 5      \\
0.884 & 10     \\
0.884 & 15     \\
0.885 & 5      \\
0.885 & 10     \\
0.885 & 15     \\
0.886 & 5      \\
0.886 & 10     \\
0.886 & 15     \\
0.887 & 5      \\
0.887 & 10     \\
0.887 & 15     \\
0.888 & 5      \\
0.888 & 10     \\
0.888 & 15     \\
0.889 & 5      \\
0.889 & 10     \\
0.889 & 15    \\
    \bottomrule
    \end{tabular}
\end{table}


The homogeneity scores of the clustering results are calculated for all values of K from 60 to 120 in the k-means cluster method, and all combinations of the parameters, shown in Table \ref{tab:dbscan_grid_search} for the DBSCAN method. The homogeneity scores are calculated for different resolution levels, i.e., L1, L2, L3, and L4 levels of power profile classification. 
For example, in section 5.1 of the paper, we report the result of k-means only for the K value, corresponding to the number of distinct labels at level-3. The number of classes at level-3 is 70 and the reason to choose the value of K. We do this because at level L4 there are over 100 classes and few datapoints in one class, contrary to that levels L1 and L2 are too coarse-grained. Thus, level L3 provides the right balance of classification based on the power profile patterns.

For prediction results, presented in section 5.2, we run the k-means clustering technique on stratified-kfold cross-validation method for different values of K. We save the homogeneity score in a matrix. Rows in a matrix correspond to class labels and columns represent the value of K. For each class/label for a value of K, we save the homogeneity score in a cell corresponding to the class label and K. 

\subsubsection{How Experiment Workflow Relate to the Results Found in the Article}
The results presented in the paper are the final outcomes of the workflow pipeline. The two main results are: 1) clustering to find the patterns exhibited by jobs running on the HPC system, and 2) prediction using the clustering methods for the jobs that have not been exposed to clustering algorithms. In the clustering approach, we apply k-means and DBSCAN. For both algorithms, the workflow is designed to run over a large search space. 
The output generated by the workflow is in the matrix. Each column of the matrix contains the labels assigned by the clustering method to the data. For k-means, the result matrix includes 60 columns and 846 rows. Each column corresponds to the value of K from 60 to 119. For DBSCAN, the output from the workflow matrix has 30 columns and 846 rows.  

The clustering results shown in the article in section 5.1 corresponds to the homogeneity score calculated on one column of the k-means matrix for which the value of $K=70$, and for the DBSCAN method, the results in the paper is from a column in the DBSCAN matrix that corresponds to parameter values $epsilon=.889$ and minimum sample per class as $mininmum\_sample=10$.
The plots in Figures 8 to 11 are the line plots of the power values and are grouped based on clustering results corresponding to column $K=70$ for the k-means matrix. For the DBSCAN matrix, the line plots are from the column corresponding to $epsilon=.889$ and $mininmum\_sample=10$.

The prediction results shown in section 5.2 is from k-means cluster after partitioning the data into 80\% for clustering and 20\% for prediction. 
The prediction output generated for different levels is stored in a matrix format. Different K values correspond to the columns and the 20\% test samples correspond to the number of rows. The value in each cell of the result matrix represents the prediction label of a sample job for a particular K value. Based on the actual number of classes in different granularity levels (L1, L2, L3, L4), we choose the K values ranging between $\pm 5$ of the actual number of classes. We calculate the homogeneity score using the real class labels and the predicted labels of all the test job samples for all K values. In Table 7 in the article, we only report the score that corresponds to the actual number of classes in levels L1, L2, L3, and L4. 

The heat-map in Figure 12 represents the class-wise homogeneity score for different values of K at four different classification levels corresponding to four heat-maps. At different classification levels, the class-wise homogeneity scores are stored in the matrix format where the number of rows is the actual classes, and the columns are different K values. These 4 output matrices are used to generate the heat-maps.

%STOP_LATEX

==> txt/future.tex <==
\section{Future work}

\subsubsection*{\textbf{TBD Future Work Item:}}
dictumst quisque sagittis purus sit amet volutpat consequat mauris nunc congue nisi vitae suscipit tellus mauris a diam maecenas sed enim ut sem viverra aliquet eget sit amet tellus cras adipiscing enim eu turpis egestas pretium aenean pharetra magna ac placerat vestibulum lectus mauris ultrices eros in cursus turpis massa tincidunt dui ut ornare lectus sit amet est placerat in egestas erat imperdiet sed euismod nisi porta lorem mollis aliquam ut porttitor leo a diam sollicitudin tempor id eu nisl nunc mi ipsum faucibus vitae aliquet nec ullamcorper sit amet risus nullam eget felis eget nunc lobortis mattis aliquam faucibus purus in massa tempor nec feugiat nisl pretium fusce id velit ut tortor pretium viverra suspendisse potenti nullam ac tortor vitae purus faucibus ornare suspendisse sed nisi lacus sed viverra tellus in hac habitasse platea dictumst vestibulum rhoncus est pellentesque elit ullamcorper dignissim cras tincidunt lobortis feugiat vivamus at augue eget arcu dictum varius duis at consectetur lorem donec massa sapien faucibus et molestie ac feugiat sed lectus vestibulum mattis ullamcorper velit sed ullamcorper morbi tincidunt ornare massa eget egestas purus viverra accumsan in nisl nisi scelerisque eu ultrices vitae auctor eu augue ut lectus arcu bibendum at varius vel

dictumst quisque sagittis purus sit amet volutpat consequat mauris nunc congue nisi vitae suscipit tellus mauris a diam maecenas sed enim ut sem viverra aliquet eget sit amet tellus cras adipiscing enim eu turpis egestas pretium aenean pharetra magna ac placerat vestibulum lectus mauris ultrices eros in cursus turpis massa tincidunt dui ut ornare lectus sit amet est placerat in egestas erat imperdiet sed euismod nisi porta lorem mollis aliquam ut porttitor leo a diam sollicitudin tempor id eu nisl nunc mi ipsum faucibus vitae aliquet nec ullamcorper sit amet risus nullam eget felis eget nunc lobortis mattis aliquam faucibus purus in massa tempor nec feugiat nisl pretium fusce id velit ut tortor pretium viverra suspendisse potenti nullam ac tortor vitae purus faucibus ornare suspendisse sed nisi lacus sed viverra tellus in hac habitasse platea dictumst vestibulum rhoncus est pellentesque elit ullamcorper dignissim cras tincidunt lobortis feugiat vivamus at augue eget arcu dictum varius duis at consectetur lorem donec massa sapien faucibus et molestie ac feugiat sed lectus vestibulum mattis ullamcorper velit sed ullamcorper morbi tincidunt ornare massa eget egestas purus viverra accumsan in nisl nisi scelerisque eu ultrices vitae auctor eu augue ut lectus arcu bibendum at varius vel
